Grounding Multimodal LLMs to Embodied Agents that Ask for Help with Reinforcement Learning

Embodied agents operating in household environments must interpret ambiguous and under-specified human instructions. A capable household robot should recognize ambiguity and ask relevant clarification questions to infer the user intent accurately, leading to more effective task execution. To study this problem, we introduce the Ask-to-Act task, where an embodied agent is tasked with a single or multi-object rearrangement task using an under-specified instruction in a home environment. The agent must strategically ask minimal, yet relevant, clarification questions to resolve ambiguity while navigating under partial observability. To address this challenge, we propose a novel approach that fine-tunes multi-modal large language models (MLLMs) as vision-language-action (VLA) policies using online reinforcement learning (RL) with LLM-generated rewards. Our method eliminates the need for large-scale human demonstrations or manually engineered rewards for training such agents. We benchmark against strong zero-shot baselines including GPT-4o as well as supervised fine-tuned MLLMs on our task. Our results show that our RL-finetuned MLLM outperforms all baselines by a significant margin (10.4-16.5%), generalizing well to novel scenes and tasks. To the best of our knowledge, this is the first demonstration of adapting MLLMs as VLA agents that can act and ask for help using LLM-generated rewards with online RL.

==> space_saver.tex <==
% A collection of dubious space saving macros
%\setlength{\parindent}{0cm}
%\parskip=2pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies

%Section spacing
\newcommand{\csection}[1]{
    \vspace{-0.08in}
    \section{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsection}[1]{
    \vspace{-0.08in}
    \subsection{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsubsection}[1]{
    \vspace{-0.06in}
    \subsubsection{#1}
    \vspace{-0.05in}
}


%caption/figure spacing
\setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
%\setlength{\textfloatsep}{0ex plus 0ex minus 0ex}
%\setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
\setlength{\belowcaptionskip}{0ex plus 0ex minus 0.5ex}

==> tables/dataset.tex <==

\resizebox{1.0\columnwidth}{!}{
  {\footnotesize
    {\renewcommand{\arraystretch}{1.2}%
      \begin{tabular}{P{0.01\columnwidth}P{0.15\columnwidth}|m{0.42\columnwidth}|m{0.42\columnwidth}}
  & \textbf{Dataset Name} & \textbf{Instruction Example} & \textbf{Description} \\
  \cmidrule{2-4}
  & \cellcolor{lightgray}Train & \cellcolor{lightgray}\emph{Find an apple and put it away in the fridge.} & \cellcolor{lightgray}Instructions used to train the agent. \\
  & New Scenes & \textit{Find an apple and put it away in the fridge} & Same instructions, but in new scenes. All other datasets are in new scenes. \\
  \cmidrule{2-4}
        \multirow{4}{0em}{\rotatebox{90}{\textbf{\paragen}}}  & \cellcolor{lightgray}Instruction Rephrasing & \cellcolor{lightgray}\textit{\change{In the fridge, stow} an apple.} & \cellcolor{lightgray}Swap the order that nouns appear in the instruction and substitute synonyms for verbs. \\
        & Referring Expressions & \textit{Find the \change{round red fruit} and put it in the fridge} & Refer to objects by their visual appearance. \\
        & \cellcolor{lightgray}Spatial Relationships & \cellcolor{lightgray}\textit{Find an apple and put it in the receptacle to the \change{right of the kitchen counter}.} & \cellcolor{lightgray}Refer to receptacles indirectly by their location relative to other receptacles. \\
        & Context & \textit{\change{I am hungry for something sweet and healthy}. Put a snack for me on the table.} & Describe a situation where a particular object fits the context. \\
        & \cellcolor{lightgray}Irrelevant Instruction Text & \cellcolor{lightgray}\textit{\change{There is a pear on the counter.} Find an apple and put it away in the fridge.} &  \cellcolor{lightgray}Instructions that include irrelevant context. \\
        \cmidrule{2-4}
        & Multiple Rearrangements & \textit{\change{Find an apple, pear, and banana} and put them away in the fridge.} & Rearrange 3 objects (2 max during training). \\
        \multirow{4}{0em}{\rotatebox{90}{\textbf{Behavior Gen.}}}                                               & \cellcolor{lightgray}Novel Objects & \cellcolor{lightgray}\textit{Find an \change{orange} and put it away in the fridge} & \cellcolor{lightgray}New entity / instruction pairs. \\
        & Multiple Objects & \textit{Put \change{all the apples} in the fridge.} & Find all of an object. \\
        & \cellcolor{lightgray}Conditional Instructions & \cellcolor{lightgray}\textit{\change{If the fridge is open}, find an apple and put it there. Otherwise put an apple on the table.} & \cellcolor{lightgray}Adjust behavior based on if the conditional statement is true.\\
        \cmidrule{2-4}
      \end{tabular}
    }
  }
}

